CrossGaze: A Strong Method for 3D Gaze Estimation in the Wild

Gaze estimation, the task of predicting where an individual is looking, is a critical task with direct applications in areas such as human-computer interaction and virtual reality. Estimating the direction of looking in unconstrained environments is difficult, due to the many factors that can obscure the face and eye regions. In this work we propose CrossGaze, a strong baseline for gaze estimation, that leverages recent developments in computer vision architectures and attention-based modules. Unlike previous approaches, our method does not require a specialised architecture, utilizing already established models that we integrate in our architecture and adapt for the task of 3D gaze estimation. This approach allows for seamless updates to the architecture as any module can be replaced with more powerful feature extractors. On the Gaze360 benchmark, our model surpasses several state-of-the-art methods, achieving a mean angular error of 9.94 degrees. Our proposed model serves as a strong foundation for future research and development in gaze estimation, paving the way for practical and accurate gaze prediction in real-world scenarios.

==> sections/5.0._Broader_Impact.tex <==
Gaze estimation is a technology that has many potential societal benefits, but we also acknowledge potential societal harms. It has the potential to reveal personal information about individuals, such as interests, emotions and health condition. Tracking an individual's gaze patterns over time could reveal their interests, which could be used, for example, for targeted advertising. Furthermore, gaze estimation could be used for surveillance purposes: an employer could use gaze estimation technology to monitor employees' productivity or adherence to safety protocols. The use of gaze estimation technology for surveillance purposes raises potential ethical and privacy concerns.

